DC-Ada: Reward-Only Decentralized Sensor Adaptation for Heterogeneous Multi-Robot Teams

Heterogeneity is a defining feature of deployed multi-robot teams: platforms often differ in sensing modalities, ranges, fields of view, and failure patterns. Controllers trained under nominal sensing can degrade sharply when deployed on robots with missing or mismatched sensors, even when the task and action interface are unchanged. We present DC-Ada, a reward-only decentralized adaptation method that keeps a pretrained shared policy frozen and instead adapts compact per-robot observation transforms to map heterogeneous sensing into a fixed inference interface. DC-Ada is gradient-free and communication-minimal: it uses budgeted accept/reject random search with short common-random-number rollouts under a strict step budget. We evaluate DC-Ada against four baselines in a deterministic 2D multi-robot simulator covering warehouse logistics, search and rescue, and collaborative mapping, across four heterogeneity regimes (H0--H3) and five seeds with a matched budget of $200{,}000$ joint environment steps per run. Results show that heterogeneity can substantially degrade a frozen shared policy and that no single mitigation dominates across all tasks and metrics. Observation normalization is strongest for reward robustness in warehouse logistics and competitive in search and rescue, while the frozen shared policy is strongest for reward in collaborative mapping. DC-Ada offers a useful complementary operating point: it improves completion most clearly in severe coverage-based mapping while requiring only scalar team returns and no policy fine-tuning or persistent communication. These results position DC-Ada as a practical deploy-time adaptation method for heterogeneous teams.

==> tables/extra_seed_h3_results.tex <==
\begin{table*}[t]
\centering
\scriptsize
\caption{Extended-seed confirmation for clean H3 mapping and search-and-rescue. This table combines the original five clean H3 seeds with five additional seeds (10 seeds total) for the main methods. Progress is coverage for mapping and rescue ratio for search-and-rescue. The all-environment main tables retain the uniform five-seed sweep; this targeted check evaluates whether the central H3 trends persist under additional seeds. Values are mean $\pm$ standard deviation across seeds.}
\label{tab:extra_seed_h3}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}llcccc@{}}
\toprule
\textbf{Environment} & \textbf{Method} & \textbf{n} & \textbf{Reward} & \textbf{Success (\%)} & \textbf{Progress} \\
\midrule
\multirow{5}{*}{Mapping} & Shared policy & 10 & \textbf{4783.0 $\pm$ 1.4} & 3.9 $\pm$ 0.1 & 0.656 $\pm$ 0.000 \\
 & DC-Ada (Ours) & 10 & 4736.6 $\pm$ 70.1 & \textbf{11.2 $\pm$ 2.4} & \textbf{0.675 $\pm$ 0.002} \\
 & Random perturbation & 10 & 4690.5 $\pm$ 51.6 & 6.0 $\pm$ 1.4 & 0.657 $\pm$ 0.005 \\
 & Local fine-tuning & 10 & 4779.7 $\pm$ 1.8 & 4.4 $\pm$ 0.2 & 0.658 $\pm$ 0.000 \\
 & Obs. normalization & 10 & 4694.6 $\pm$ 0.9 & 0.0 $\pm$ 0.0 & 0.624 $\pm$ 0.000 \\
\midrule
\multirow{5}{*}{Search--Rescue} & Shared policy & 10 & \textbf{16.05 $\pm$ 0.08} & 12.5 $\pm$ 0.1 & 0.299 $\pm$ 0.001 \\
 & DC-Ada (Ours) & 10 & 14.42 $\pm$ 1.36 & 13.4 $\pm$ 2.0 & 0.290 $\pm$ 0.021 \\
 & Random perturbation & 10 & 13.45 $\pm$ 1.51 & \textbf{13.8 $\pm$ 1.4} & \textbf{0.307 $\pm$ 0.016} \\
 & Local fine-tuning & 10 & 14.67 $\pm$ 0.11 & 11.8 $\pm$ 0.2 & 0.290 $\pm$ 0.002 \\
 & Obs. normalization & 10 & 15.94 $\pm$ 0.14 & 10.5 $\pm$ 0.3 & 0.291 $\pm$ 0.002 \\
\bottomrule
\end{tabular*}
\end{table*}
